Optimal Sufficient Requirements on the Embedded Ising Problem in Polynomial Time

One of the central applications for quantum annealers is to find the solutions of Ising problems. Suitable Ising problems, however, need to be formulated such that they, on the one hand, respect the specific restrictions of the hardware and, on the other hand, represent the original problems which shall actually be solved. We evaluate sufficient requirements on such an embedded Ising problem analytically and transform them into a linear optimization problem. With an objective function aiming to minimize the maximal absolute problem parameter, the precision issues of the annealers are addressed. Due to the redundancy of several constraints, we can show that the formally exponentially large optimization problem can be reduced and finally solved in polynomial time for the standard embedding setting where the embedded vertices induce trees. This allows to formulate provably equivalent embedded Ising problems in a practical setup.

==> adds/Statements.tex <==

\section*{Statements and Declarations}

\subsection*{Funding}

The authors declare that no funds, grants, or other support were received during the preparation of this manuscript.

\subsection*{Competing Interests}

The authors have no relevant financial or non-financial interests to disclose.

% \subsection{Author Contributions}
% 
% All authors contributed to the study conception and design. Material preparation, data collection and analysis were performed by [full name], [full name] and [full name]. 
% The first draft of the manuscript was written by [full name] and all authors commented on previous versions of the manuscript. All authors read and approved the final manuscript.


==> adds/letter.tex <==

work based on my dissertation 

slight restructuring due to extraction of preliminaries

improved proof of the final due to simpler notation


==> modules/Weight_Distribution/content/problem/simplifications/cuts.tex <==

%

\subsubsection{Graph Cuts}

With the former simplifications, we can now further evaluate the condition 
\begin{multline}
    \quad I_{\omega, \vartheta}^\sigma(r, s) \geq \min \left\{I_{\omega, \vartheta}^\sigma(-\One, s), I_{\omega, \vartheta}^\sigma(\One, s) \right\} + \gamma
        \ifjournalversion{\\}{\quad}\forall s \in \{-1,1\}^\vertices ~\forall r \in \{-1,1\}^\vertices \setminus \{-\One, \One\} \quad
\end{multline}
for fixed parameters and reformulate it using graph cuts. 
Inserting the full formulation for $I_{\omega, \vartheta}^\sigma$, we have for all $s \in \{-1,1\}^\vertices$ and for all $r \in \{-1,1\}^\vertices \setminus \{-\One, \One\}$:   
\begin{alignat}{2}
    &&&\sum_{q \in \vertices} \omega_q r_q - \vartheta \sum_{pq \in \edges} r_p r_q + \sum_{q \in \vertices} \sigma_q r_q s_q \\
        &\geq{}&&\min \left\{ \sum_{q \in \vertices} \omega_q (-1) - \vartheta \sum_{pq \in \edges} (-1)(-1) + \sum_{q \in \vertices} \sigma_q s_q (-1),\, 
                           \sum_{q \in \vertices} \omega_q - \vartheta \sum_{pq \in \edges} 1 + \sum_{q \in \vertices} \sigma_q s_q \right\} + \gamma\\
        &= &&\min \left\{- \sum_{q \in \vertices} (\sigma_q s_q + \omega_q),\, \sum_{q \in \vertices} (\sigma_q s_q + \omega_q)\right\} - \vartheta|\edges| + \gamma,
\end{alignat}
which is equivalent to
\begin{align}
    \vartheta|\edges| - \vartheta\sum_{pq \in \edges} r_p r_q &= \vartheta\bigg(|\edges| - \sum_{pq \in \edges} r_p r_q \bigg) \\
        &= \vartheta\big(|\edges| - |\{pq \in \edges : r_p = r_q\}| + |\{pq \in \edges : r_p = - r_q\}|\big) \\
        &= 2\vartheta |\{pq \in \edges : r_p = - r_q\}|\\
        &\geq \min \left\{\sum_{q \in \vertices} (\sigma_q s_q + \omega_q) ,\, - \sum_{q \in \vertices} (\sigma_q s_q + \omega_q)\right\} - \sum_{q \in \vertices} (\sigma_q s_q + \omega_q) r_q + \gamma\\
        &= \min \left\{\sum_{q \in \vertices}  (\sigma_q s_q + \omega_q) (1 - r_q), \, \sum_{q \in \vertices} (\sigma_q s_q + \omega_q) (- 1 - r_q) \right\} + \gamma\\
        &= 2\min \Biggl\{~\sum_{\substack{q \in \vertices \\ \mathclap{r_q = -1}}} (\sigma_q s_q + \omega_q), \, - \sum_{\substack{q \in \vertices \\ \mathclap{r_q = 1}}} (\sigma_q s_q + \omega_q)\Biggr\} + \gamma.
\end{align}

By combining all the lower bounds, we can further deduce stronger conditions, where we have for all $r \in \{-1,1\}^\vertices \setminus \{-\One, \One\}$:
\begin{align}
    \vartheta |\{pq \in \edges : r_p = - r_q\}| &\geq \max_{s \in \{-1, 1\}^\vertices} \min \Biggl\{~ \sum_{\substack{q \in \vertices \\ \mathclap{r_q = -1}}}  (\sigma_q s_q + \omega_q), \,
                                                                                    - \sum_{\substack{q \in \vertices \\ \mathclap{r_q = 1}}}  (\sigma_q s_q + \omega_q)\Biggr\} + \tfrac{1}{2}\gamma\\
    &= \min \Biggl\{~\sum_{\substack{q \in \vertices \\ \mathclap{r_q = -1}}} (\sigma_q + \omega_q), \sum_{\substack{q \in \vertices \\ \mathclap{r_q = 1}}} (\sigma_q - \omega_q)\Biggr\} + \tfrac{1}{2}\gamma.
\end{align}
It is easy to recognize that the maximum in the former relation is achieved when setting $s_q$ to~$-r_q$ for all $q \in \vertices$, leading to the last equality.
Note that we already reduced the number of constraints to $2^{|\vertices|} - 2$ with this step. 

With the vertex set definition of $S = \{q \in \vertices : r_q = -1\}$ for a specific assignment of the $r$-variables and 
\begin{equation}
    \pmb{\sigma(S)} \vcentcolon = \sum_{q \in S} \sigma_q, 
\end{equation}
we can equivalently formulate for all $\emptyset \neq S \subsetneq \vertices$: 
\begin{align}
    \vartheta |\{pq \in \edges : p \in S, q \in \vertices \setminus S\}| = \vartheta|\delta(S)|
            &\geq \min \Biggl\{\sum_{q \in S} (\sigma_q + \omega_q), \sum_{q \in \vertices \setminus S} (\sigma_q - \omega_q)\Biggr\} + \tfrac{1}{2}\gamma\\
            &= \min \big\{\sigma(S) + \omega(S), \sigma(\vertices \setminus S) - \omega(\vertices \setminus S)\big\} + \tfrac{1}{2}\gamma.
\end{align}
Note that the empty set and the full vertex set are excluded 
because the $r$-variables cannot get all the value $1$ or all the value $-1$.
As furthermore the graph $H[\varphi_v]$ is connected by the embedding definition, we have $|\delta(S)| > 0$ for all non-trivial cuts $S$. 
As $\vartheta$ is the objective function, we can reformulate the conditions to lower bounds on the optimal value with 
\begin{equation}
    \vartheta \geq \frac{\min \{\sigma(S) + \omega(S), \sigma(\vertices \setminus S) - \omega(\vertices \setminus S)\} + \tfrac{1}{2}\gamma}{|\delta(S)|} \quad \forall \emptyset \neq S \subsetneq \vertices. 
\end{equation}
We refer to them as \emph{cut inequalities} in the following. 
They can equivalently be combined all in one with 
\begin{equation}
    \vartheta \geq \max_{\emptyset \neq S \subsetneq \vertices}\left\{\frac{\min \{\sigma(S) + \omega(S), \sigma(\vertices \setminus S) - \omega(\vertices \setminus S)\}+ \tfrac{1}{2}\gamma}{|\delta(S)|} \right\}.  
\end{equation}

Note that, according to the preprocessing step based on \autoref{lem:preprocess} of \autoref{sec:ising}, 
there are instances for which the weight of the original vertex predominates all outer influences caused by its incident edges.
The variable corresponding to such a vertex can be preprocessed before the embedding anyway
by setting it according to the sign of the weight.  
This case appears if we have $\totalweight \geq \sigma(\vertices)$. 
Thus, we also only consider instances with $\sigma(\vertices) > \totalweight$ in the following.
We summarize the resulting problem in the next section. 

%


==> modules/Weight_Distribution/content/problem/simplifications/independent.tex <==

%
     
\subsubsection{Independent Outer Neighbors}
%

By the embedding definition, a single edge connecting the embeddings of different vertices is sufficient. 
In practice, we usually have $|\delta_{vw}| > 1$ for at least a few pairs of original vertices $vw$ due to the symmetric structure of the Chimera. 
This can also be seen in \autoref{fig:subgraph}. 
Here, we discuss some options and the assumptions which we base the following work on. 

If there are multiple edges between the embeddings of two vertices, 
one possibility could simply be to choose a certain edge $\bar{e} \in \delta_{vw}$ and `ignore' the others. %
This means, for the embedded Ising model, we could set
\begin{equation}
\begin{aligned}
    \alpha_{\bar{e}} = \closure{S}_{\bar{e}} & \vcentcolon = S_{vw}, \\
    \alpha_{e} = \closure{S}_{e} & \vcentcolon = 0 &&\forall e \in \delta_{vw} \setminus \{\bar{e}\}
\end{aligned}
\end{equation}
and further only deal with $\delta_{vw} = \{\bar{e}\}$.  
This would influence the former graph structure in two ways: 
\begin{enumerate}
    \item\label{item:no_share} No two vertices of $\vertices$ share an outer neighbor, 
          which means \ifjournalversion{that}{} we have $|\{q : qn \in \delta(\varphi_v)\}| = 1$ for all $n \in \outerneighbors$ and thus $\outeredges = \delta(\varphi_v) \cong \outerneighbors$. 
          %
    \item\label{item:no_edge} We have $E(H[N(\varphi_v)])) = \emptyset$, which means that no two outer neighbors are connected by an edge. 
\end{enumerate}
%
By this, on the one hand, we have already achieved a simplification of the problem and, 
on the other hand, we have ensured that all the outer neighbors are independent of each other 
because they belong to different original neighbors of $v$. 

%
%
%
%
%
%
%

However, another possibility also offers advantages: 
By spreading the strength equally over all of the available edges as suggested in \cite{raymond2020improving} with 
\begin{equation}
    \alpha_{pq} = \closure{S}_{pq} \vcentcolon = \frac{S_{vw}}{|\delta_{vw}|} \qquad \forall pq \in \delta_{vw},
\end{equation}
the coefficients are decreased as much as possible. 
This seems to be beneficial for complying with the parameter range of the machine.
%
As the variables corresponding to the embeddings of the other vertices shall be synchronized, too, 
the outer neighbors of some inner vertices are not independent of each other in this case. 
While in the Chimera graph no triangles exist, 
they might be present in other hardware graphs, such as the Pegasus graph, 
and might cause inner vertices that even share a common outer neighbor. 

Howsoever the strengths are distributed, we want to take advantage of both strategies. 
Thus, we simplify the embedded graph structure by splitting up possibly existing shared vertices 
and simply considering all outer vertices to be pairwise independent of each other 
as if they would belong to different neighbors of the original vertex. 
Thus, for the following considerations in this work, we assume that we have $\outeredges \cong \outerneighbors$
and that $\pmb{\alpha} \in \R_{\geq 0}^\outeredges = \R_{\geq 0}^\outerneighbors$ are given and fixed strengths 
yielding the points \ref{item:no_share} and \ref{item:no_edge} from above. 

These assumptions become relevant in the following section, where we estimate the worst cases of the `outer influence', 
the contribution of the strengths on the edges to the outer neighbors multiplied by the $s$-variables, 
to further simplify $\closure{I}\vphantom{I}^v$.
If there exist two variables $s_n$ and $s_m$ corresponding to two outer neighbors $n,m \in \outerneighbors$ 
that belong to the same embedding $\varphi_w$ of an original neighboring vertex $w$, 
those variables would get the same value in a synchronized solution of the overall problem. 
As we however assume they can be chosen arbitrarily and independently, 
the worst case might be overestimated. 
This means our derived bounds still hold,
but the found strength might be larger than actually necessary in this case.  
Additionally, the actual minimal gap between a synchronized and an unsynchronized solution might be larger than intended by the user. 
This is another point where we can only derive the sufficiency but not the necessity of our conditions.


%


==> modules/Weight_Distribution/content/problem/simplifications/single.tex <==

%

\subsubsection{Single Outer Neighbor}
        
Finally, we further reduce the problem such that the given graph instance does only have a single outer neighbor for each vertex $q \in \vertices$. 
This would mean we had $\outerneighbors \cong \vertices$. 
If this is not the case, which means there are at least two outer neighbors for a single inner vertex,
the following lemma shows that a synchronization of the variables over these outer neighbors suffices 
to also cover those cases where the strengths on the outer edges get different signs.

\begin{lemma}
    For $I_{\omega, \vartheta}^\alpha : \{-1, 1\}^\vertices \times \{-1, 1\}^\outerneighbors$ as given in \eqref{eq:ising} with $\alpha \in R_{\geq 0}^\outeredges$, the gap value $\gamma \in \R_{\geq 0}$,
    a vertex $q \in \vertices$ and its neighbors $n, m \in \outerneighbors$ with $qn, qm \in \outeredges$, we have   
    \begin{equation}
    \begin{aligned}
        &I_{\omega, \vartheta}^\alpha(r, s) \geq \min \left\{I_{\omega, \vartheta}^\alpha(-\One, s), I_{\omega, \vartheta}^\alpha(\One, s) \right\} + \gamma &&\text{for } s_n = s_m \in \{-1, 1\}\\ 
        \Rightarrow~ &I_{\omega, \vartheta}^\alpha(r, s) \geq \min \left\{I_{\omega, \vartheta}^\alpha(-\One, s), I_{\omega, \vartheta}^\alpha(\One, s) \right\} + \gamma &&\text{for } s_n, s_m \in \{-1, 1\}
    \end{aligned}   
    \end{equation}  
    for all $r \in \{-1, 1\}^\vertices$ and all $s_{\outerneighbors \setminus \{m, n\}} \in \{-1, 1\}^{\outerneighbors \setminus \{m, n\}}$.   
\end{lemma}
\begin{proof}
    In the following proof, we drop the sub- and superscripts on $I$ for simplicity.  
    With 
    \begin{align}
        I(r, s) &= &\hspace{-0.8em}\alpha_{qn} s_n r_q + \alpha_{qm} s_m r_q \ifjournalversion{}{&}- \vartheta|\edges| + \gamma
                     + r_q \bigg(\!\underbrace{\omega_q - \vartheta\!\! \sum_{pq \in \edges} r_p  + \sum_{\substack{q\ell \in \outeredges \\ \ell \neq n,m}} \alpha_{q\ell} s_\ell}_{=\vcentcolon A(r,s)}\!\bigg) \\
                     &&\ifjournalversion{}{&\,}+ \underbrace{\vartheta|\edges| - \gamma + \sum_{p \in \vertices \setminus \{q\}} \omega_p r_p - \vartheta\!\! \sum_{\substack{pu \in \edges \\ p,u \neq q}} r_p r_u + \sum_{p \in \vertices\setminus\{q\}} \sum_{p\ell \in \outeredges} \alpha_{p\ell} s_\ell r_p}_{=\vcentcolon B(r,s)} \\[-1.5\baselineskip]
    \end{align}
    and 
    \begin{equation}
        I(\pm\One, s) = \pm \bigg(\alpha_{qn} s_n + \alpha_{qm} s_m + \underbrace{\sum_{\substack{p\ell \in \outeredges \\ \ell \neq n,m}} \alpha_{p\ell} s_\ell + \totalweight}_{= \vcentcolon C(r, s)} \bigg) - \vartheta|\edges| + \gamma,
    \end{equation}
    the functions $A$, $B$ and $C$ are independent of $r_q$, $s_n$ and $s_m$. 
    By the condition of the lemma, we know 
    \begin{align}
         &\alpha_{qn} s_n r_q + \alpha_{qm} s_m r_q + A(r, s) r_q + B(r, s) \geq - \big| \alpha_{qn} s_n + \alpha_{qm} s_m + C(r, s)\big| \\
            &\qquad\forall s_n {\color{lightgreen}{}\pmb{=}{}} s_m \in \{-1,1\} ~\forall r_q \in \{-1,1\} ~\ifjournalversion{\\ &\qquad}{}\forall s \in \{-1,1\}^{\outerneighbors \setminus \{n, m\}} ~\forall r \in \{-1,1\}^{\vertices \setminus \{q\}} \setminus \{-\One, \One\}\phantom{.}
    \end{align}
    and it remains to show that from this follows 
    \begin{align}
         &\alpha_{qn} s_n r_q + \alpha_{qm} s_m r_q + A(r, s) r_q + B(r, s) \geq - \big| \alpha_{qn} s_n + \alpha_{qm} s_m + C(r, s)\big| \\
            &\qquad\forall s_n {\color{darkgreen}{}\pmb{\neq}{}} s_m \in \{-1,1\} ~\forall r_q \in \{-1,1\} ~\ifjournalversion{\\ &\qquad}{}\forall s \in \{-1,1\}^{\outerneighbors \setminus \{n, m\}} ~\forall r \in \{-1,1\}^{\vertices \setminus \{q\}} \setminus \{-\One, \One\}.
    \end{align}
    
    More simply, this means to show that, for any fixed $A, B, C \in \R$ and $X, Y \in \R_{\geq 0}$ with 
    \begin{equation}
        (X + Y) s r + A r + B \geq - | (X + Y) s + C| \qquad\forall r, s \in \{-1,1\}, \label{eq:have}
    \end{equation}
    it follows that
    \begin{equation}
        (X - Y) s r + A r + B \geq - | (X - Y) s + C| \qquad\forall r, s \in \{-1,1\}.  \label{eq:toshow}
    \end{equation}
    This can be achieved by the following two case distinctions. 
    By inserting $s=-1$ and $r=1$ in inequality \eqref{eq:have}, we obtain due to $X, Y \geq 0$   
    \begin{itemize}%
        \item for $C \leq X + Y$
            \begin{align}  
                &&- X - Y + A + B  &\geq - | -(X + Y) + C| = - X - Y + C \\
                &\Leftrightarrow & A + B  &\geq C \\
                &\Leftrightarrow~ & (X - Y) s + A + B  &\geq (X - Y) s + C \\
                    &&&\geq - |(X - Y) s + C| &&\negthickspace\forall s \in \{-1, 1\}
        \intertext{\item and for $C > X + Y$}
            &&- X - Y + A + B &\geq - | -(X + Y) + C| = X + Y - C \\
            &\Rightarrow& (X - Y) s  + A + B &\geq - X - Y + A + B  \\
                                        &&&\geq X + Y - C \\
                                        &&&\geq -(X - Y) s - C \\
                                        &&&\geq - |(X - Y) s + C| &&\negthickspace\forall s \in \{-1, 1\}.
        \end{align} 
    \end{itemize}
    Thus, we have shown the implication of inequality \eqref{eq:toshow} for r = 1 and arbitrary s.
    By inserting $s=1$ and $r=-1$ in inequality \eqref{eq:have}, we obtain in turn 
    \begin{itemize}
        \item for $C \geq -X - Y$
        \begin{align}
            &&- X - Y - A + B  &\geq - | X + Y + C| = - X - Y - C\\
            &\Leftrightarrow & -A + B  &\geq -C \\
            &\Leftrightarrow~ & -(X - Y) s -A + B  &> -(X - Y) s - C \\
                                        &&&\geq - |-(X - Y) s - C| \\
                                        &&&= - |(X - Y) s + C| &&\forall s \in \{-1, 1\}
        \intertext{\item and for $C < -X - Y$}
            &&- X - Y - A + B  &> - | X + Y + C| = X + Y + C \\
            &\Rightarrow &-(X - Y) s  - A + B &\geq - X - Y - A + B  \\
                                        &&&\geq X + Y + C \\
                                        &&&\geq (X - Y)s + C \\ 
                                        &&&\geq - |(X - Y) s + C|  &&\forall s \in \{-1, 1\}.
        \end{align}
    \end{itemize}%
    This means we have also shown implication of inequality \eqref{eq:toshow} for $r = -1$ and arbitrary $s$, which completes the proof. 
\end{proof}

With the conditions of the lemma, we can replace the single occurrence of $s_m$ with $s_n$ in $I_{\omega, \vartheta}^\alpha(r, s)$. 
This way $s_n$ gets the coefficient $\alpha_{qn} + \alpha_{qm}$ and we have reduced the outer neighbors by 1 by removing~$m$. 
We can apply this lemma iteratively to all outer neighbors that share an inner vertex. 
Hence, by the lemma, we can say that the synchronization of the variables corresponding to the outer neighbors forms the `worst case' with respect to the outer influence.   
By defining the weighting $\pmb{\sigma} \in \R_{\geq 0}^\vertices$ with
\begin{equation}
    \pmb{\sigma_q} \vcentcolon = \sum_{qn \in \outeredges} \alpha_{qn} \quad \forall q \in \vertices,
\end{equation}
we can therefore reduce the Ising model to 
\begin{equation}
    \pmb{I_{\omega, \vartheta}^\sigma(r, s)} = \sum_{q \in \vertices} \omega_q r_q - \vartheta \sum_{pq \in \edges} r_p r_q + \sum_{p \in \vertices} \sigma_q r_q s_q,   
\end{equation}
where we reindexed the $s$-variables accordingly, that is $s \in \{-1, 1\}^{\vertices}$.  
Thus, only $\sigma \in \R_{\geq 0}^\vertices$ is considered in the following as an input for the weight distribution problem
and we do not require the outer neighbors $\outerneighbors$ and the edges to them $\outeredges$ anymore.

%


==> modules/Weight_Distribution/content/problem/simplifications/strength.tex <==

%

\subsubsection{Common Strength}

The $\beta$-variables only introduce an offset for synchronized variable assignments.  
As the total size of this offset is irrelevant, we can choose to set all strengths to the same maximal value.  
Thus, with $\pmb{\vartheta} \vcentcolon = \|\beta \|_\infty$, we can set $\beta_{pq}$ to $\vartheta$ for all $pq \in \edges$ and therefore get
\begin{equation}\label{eq:ising}
    I_{\omega, \vartheta}^{\alpha}(r,s) = \sum_{q \in \vertices} \omega_q r_q - \vartheta \sum_{pq \in \edges} r_p r_q + \sum_{q \in \vertices} \sum_{qn \in \outeredges} \alpha_{qn}r_q s_n. 
\end{equation}
The constant $c$ describing the difference to the original Ising model is now simply~$\vartheta|\edges|$. 

This also allows to further simplify the problem formulation: 
Instead of using $\max\big\{\|\omega\|_\infty, \vartheta\big\}$ as the objective function to be minimized,
it can be reduced to only $\vartheta$
by introducing the additional constraint $\vartheta \geq \|\omega\|_\infty$.
This means the minimal coupling strength also serves as an upper bound for the weights which we can assign. 

%


==> modules/Weight_Distribution/content/problem/simplifications/summary.tex <==

%
\subsection{The Problem}\label{sec:probs}

In this section, we briefly summarize the problem that is derived from \refProb{original}, 
where the sufficient requirements on the embedded Ising Problem are combined. 
Previously, we have considered a more complex objective function, which has now been reduced to simply optimize $\vartheta$ while distributing the weights~$\omega$. 
Therefore, we have

\begin{fprob*}[\textsc{Gapped Weight Distribution Problem}]\label{prob:both}
    Given a graph $G = (V, E)$, $\sigma \in \R_{\geq 0}^V$, $\totalweight \in \R_{\geq 0}$ with $\totalweight < \sigma(V)$ and $\gamma \in \R_{>0}$, find $\vartheta$ and $\omega$ that solve
    \begin{equation}
    \begin{aligned}
        \min~        &\vartheta  \\
        \text{s.t. } &\vartheta \in \R,\, \omega \in \R^V, \\
                     &\vartheta \geq \frac{\min \big\{\sigma(S) + \omega(S), \sigma(V \setminus S) - \omega(V \setminus S)\big\} + \gamma}{|\delta(S)|} &&\forall\emptyset \neq S \subsetneq V, \\
                     &\omega(V) = \totalweight, \\
                     &\vartheta \geq \|\omega\|_\infty.
    \end{aligned}
    \end{equation}
\end{fprob*}

Note that we have now switched to the standard notation of a graph $G = (V, E)$ as the input for \refProb{both} for simplification.
This graph $G$ does however not correspond to the interaction graph of the original Ising problem, which we introduced in the beginning of this article.
By solving the above problem with $G = H[\varphi_v]$, 
\begin{equation}
    \sigma_q = \sum_{pq \in \delta(\varphi_v)} \left|\closure{S}_{pq}\right| \quad \forall q \in \varphi_v,
\end{equation}
and $\totalweight = |W_v|$, we can find the corresponding optimal strength and weights for vertex $v$ in the embedded problem.
Thus, to get the full \refProbNamed[]{embising}, we need to repeat the optimization for all vertices and their corresponding subgraph structures and combine the results. 

Additionally, we have also substituted $\tfrac{1}{2}\gamma$ with $\gamma$ in the problem for simplicity.
This means that the actual distance between a synchronized and a non-synchronized solution is $2\gamma$ in the end.
Furthermore, note the restriction $\totalweight < \sigma(V)$, which results from \autoref{lem:preprocess} and is the reformulation of \eqref{eq:unpreprocessable} with the new notation.
It is important in the next section.

Just considering the cut constraints, we can see a relation to a graph property called the \emph{edge expansion} of the graph~\cite{hoory2006expander}. 
In our case, we additionally have a weighting $\sigma$ on the vertices, rather than just counting the number of vertices. 
This is in turn closely related to the \emph{minimum cut density} as introduced in \cite{matula1990sparsest}.
There the authors show that, in case of trees, the minimum cut density can be solved by just evaluating those partitions which are derived from cutting at each edge.
Thus, the problem can be solved in a time quadratically in the number of vertices if the examined graph is a tree. 
Although our problem formulation is slightly different to both mentioned ones, we can establish a similar results for our problem. 

%


==> modules/Weight_Distribution/content/problem/simplifications/symmetry.tex <==

%

\subsubsection{Non-negative Input Parameters Due to Symmetry}

Furthermore, we can take advantage of the symmetry in the Ising model being defined over variables in $\{-1, 1\}$.
By replacing $s$ with $\bar{s} = -s$, we can switch the sign of the strengths on the intra-coupling edges: 
\begin{equation}
\begin{aligned}
    I_{\omega, \vartheta}^{\alpha}(r,s) &= \sum_{q \in \vertices} \omega_q r_q - \vartheta \sum_{pq \in \edges} r_p r_q + \sum_{q \in \vertices} \sum_{qn \in \outeredges} \alpha_{qn} r_q s_n \\
        &= \sum_{q \in \vertices} \omega_q r_q - \vartheta \sum_{pq \in \edges} r_p r_q + \sum_{q \in \vertices} \sum_{qn \in \outeredges} (-\alpha_{qn}) r_q \bar{s}_n \\
        &= I_{\omega, \vartheta}^{-\alpha}(r, \bar{s}).
\end{aligned}
\end{equation}
We can see that the different assignments of the $s$-variables in \eqref{eq:constraint} cover all possible sign combinations of the strengths $\alpha$.    
Thus, we can restrict $\alpha$ to $\R_{\geq 0}^\outeredges$ in the following evaluations. 

Additionally, by replacing $(r, s)$ with $(\bar{r}, \bar{s})$, we observe a symmetry for the $\omega$'s: We have
\begin{equation}
\begin{aligned}
    I_{\omega, \vartheta}^{\alpha}(r,s) &= \sum_{q \in \vertices} \omega_q r_q - \vartheta \sum_{pq \in \edges} r_p r_q + \sum_{q \in \vertices} \sum_{qn \in \outeredges} \alpha_{qn} r_q s_n \\
        &= \sum_{q \in \vertices} (-\omega_q) \bar{r}_q - \vartheta \sum_{pq \in \edges} \bar{r}_p \bar{r}_q + \sum_{q \in \vertices} \sum_{qn \in \outeredges} \alpha_{qn} \bar{r}_q \bar{s}_n \\
        &= I_{-\omega, \vartheta}^{\alpha}(\bar{r}, \bar{s})
\end{aligned}
\end{equation} 
with
\begin{equation}
    \sum_{q \in \vertices} (-\omega_q) = - \totalweight.
\end{equation}
This means we can analogously restrict the total weight to $\totalweight \in \R_{\geq 0}$. 

%

